XR-penter: Material-Aware and In Situ Design of Scrap Wood Assemblies

Woodworkers have to navigate multiple considerations when planning a project, including available resources, skill-level, and intended effort. Do it yourself (DIY) woodworkers face these challenges most acutely because of tight material constraints and a desire for custom designs tailored to specific spaces. To address these needs, we present XR-penter, an extended reality (XR) application that supports in situ, material-aware woodworking for casual makers. Our system enables users to design virtual scrap wood assemblies directly in their workspace, encouraging sustainable practices through the use of discarded materials. Users register physical material as virtual twins, manipulate these twins into an assembly in XR, and preview cuts needed for fabrication. We conducted a case study and feedback sessions to demonstrate how XR-penter supports improvisational workflows in practice, the type of woodworker who would benefit most from our system, and insights on integrating similar spatial and material considerations into future work.

==> xx.tex <==
% \section{Preliminary Evaluation}
% \label{evaluation}
% % In this section, we evaluate 

% For this, we collaborated with a DIY woodworker who has 10 years of experience in self taught. <give details>
% We gave him our system and asked him to design DIY project.
% We acquired scrap materials from XX vendors
% We asked them to design improvisational objects. 

% Then came up and built these objects:

% DIY Expert interview:
% We also recruited 3 people .for the sake of resources (material and time), 

% We re-interviewed the people. We showed them the things that the DIY woodworker built with our XR system. We also showed them the video footage of the process. and walked them through the system to help them understand. We collected feedback via semi-structured interviews and formulated insights: 


% To understand how ..., we conducted a ...

% \hl{<I added placeholder stuff below to give you a sense of ho it could look, please adjust everything as you go/like:)>}

% % participants
% \subsection{Methods}

% \vspace{0.2cm} \noindent
% \textit{\textbf{Participants}}.
% We recruited 8 participants (6 male, 1 female, 1 preferred not to disclose) between the ages of 25-45. All were fluent English speakers (4 native), were regular shoppers, and all but 1 had used smartphone-based AR at least once.

% % scenario & tasks

% % \subsection{Scenario \& Tasks}

% \vspace{0.2cm} \noindent
% \textit{\textbf{Task \& Procedure}}.
% %We designed a scenario consisting of a simulated grocery shopping experience (\autoref{fig:study-setup}a) followed by an at-home experience (\autoref{fig:study-setup}b) in which users complete a set of 6 tasks using either \systemName~ or Chatbot. The task categories included: (\textbf{T1}) 2-object Search, (\textbf{T2}) N-object Search, (\textbf{T3}) Share Object, (\textbf{T4}) Get Info (Single Object), (\textbf{T5}) Set/Anchor Timer, and (\textbf{T6}) Create/Anchor Note. We created two variants of this scenario (\textbf{A} and \textbf{B}), each with the same categories but slightly varied tasks. The full set of tasks is presented in \autoref{tab:study-tasks}. 
% We designed a scenario consisting of a simulated grocery shopping experience (\autoref{fig:study-setup}a) followed by an at-home experience (\autoref{fig:study-setup}b) in which users complete a set of 6 tasks using either \systemName~ or Chatbot. \new{The tasks (\textbf{T1}-\textbf{T6}) are listed in \autoref{tab:study-tasks}, and included retrieving/comparing information about multiple objects, sharing objects, and anchoring widgets. % to objects.
% }



% First, participants were first given a brief introduction to the study, provided informed consent, and filled out a demographics survey. The experimenter then walked through the functionality of both \systemName~ and Chatbot, and participants then completed a set of sample tasks on an object not included in the study.


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figures/F6study-setup.png}
%   \caption{User study setup with mock grocery store (a) and at-home (b) environments. Examples of using \systemName~ in each case are shown in (c) and (d), respectively.}
%   \Description{(a) Shelves wıth multiple products. (b) A small table with a mug and a can. (c) A phone shows the objects on the shelf in the UI. (d) The same UI looking at the objects on the table.}
%   \label{fig:study-setup}
% \end{figure}


% Each participant completed the tasks in both scenarios \textbf{A} and \textbf{B}. The ordering of both condition (\systemName, ~Chatbot) and scenario (\textbf{A},~\textbf{B}) were counterbalanced between participants to prevent ordering effects. Once the tasks were completed, participants were free to use the tool freely for up to five additional minutes however they chose. Participants then completed a post-condition survey on their qualitative experience. %(Appendix \ref{post-condition survey}).

% After a two minute break, this was repeated with the remaining condition and scenario. Upon completing the tasks with both conditions, participants completed a final survey comparing interactions with \systemName~ and Chatbot (Appendix \ref{post-study survey}). Overall, the study took approximately 45 minutes.

% % \subsection{Measures}
% \vspace{0.2cm} \noindent
% \textit{\textbf{Measures}}.
% % \subsubsection{Task Completion Time}
% As one of our measures, we recorded the \textbf{time required to complete tasks} \textbf{T1}-\textbf{T6} for each condition as a measure of overall system performance.
% <what else?>



% \subsection{Qualitative Feedback}
% \new{We provide key insights from the responses that participants provided in their completed surveys.}

% % qualitative insights, for example, in the form of interviews or open questions

% \vspace{0.2cm} \noindent
% \new{\textit{\textbf{Helpfulness \& Efficiency}}.
% Users valued the system's streamlined interactions:
% \textit{"It saves me from looking up info myself... I just ask and it finds the info for me"} (P1).
% \textit{"Object selection and comparison was very intuitive; it was easy to get information in exactly the context I needed"} (P3).}

% \vspace{0.2cm} \noindent
% \new{\textit{\textbf{Comparative Advantage}}.
% The direct comparison with existing solutions like \textit{Google Lens} and traditional LLMs was enlightening: 
% \textit{"I was able to complete the same tasks much faster + easier"} (P1).
% \textit{"This has a lot more options, and is more flexible [in] what information it can provide"} (P2).
% \textit{"Comparing products is very helpful... less wordy than [Chatbot] and gives an answer"} (P2).}

% \vspace{0.2cm} \noindent
% \new{\textit{\textbf{Possibilities for UX Improvement}}.
% Several participants pointed out ergonomic challenges, e.g., the need to hold the phone at eye level, which informs future glass interactions as discussed in Section~\ref{discussion}:






% % \subsubsection{Study Design}
% % User studies involving both novice and experienced woodworkers were conducted to evaluate interaction effectiveness and system intuitiveness.

% % \subsubsection{Findings and Improvements}
% % Feedback from these studies influenced several refinements, improving material alignment accuracy and user interface intuitiveness.


% %To assess the effectiveness and usability of \systemName, we conducted a comprehensive user study with a diverse group of woodworkers ranging from amateurs to experienced professionals. The primary goals of this evaluation were to measure the system's impact on workflow efficiency, material utilization, user satisfaction, and overall creativity in woodworking projects.

% %\paragraph{Methodology}
% %Participants were asked to complete a series of tasks involving both traditional woodworking techniques and tasks using \systemName. These tasks were designed to compare the traditional process with the MR-enhanced process in terms of time efficiency, accuracy, ease of use, and satisfaction. Each participant completed the tasks in a controlled environment where we could monitor interactions and gather qualitative feedback through structured interviews and quantitative data through task completion times and error rates.

% %\paragraph{Metrics}
% %We used the following metrics to evaluate the performance of \systemName:

% %Time Efficiency: The time taken to complete a standard set of woodworking tasks with and without \systemName.
% %Accuracy: Measurement of the precision of cuts and fittings in the final products.
% %Ease of Use: Rated on a Likert scale based on participants’ responses to survey questions regarding their experience using the system.
% %User Satisfaction: Also rated on a Likert scale, reflecting participants' overall contentment with the process and the outcomes. 



% %\paragraph{Results}
% %The results indicated significant improvements in several areas when using \systemName:

% %Time Efficiency: Participants completed tasks up to XX\% faster using \systemName compared to traditional methods.

% %Accuracy: There was a noticeable increase in the precision of cuts, with fewer errors and adjustments needed during the task.

% %Ease of Use: Participants reported an average ease of use rating of XX out of 5, highlighting the system's intuitive design and user-friendly interface.

% %User Satisfaction: The satisfaction ratings averaged XX out of 5, with participants noting particularly how the real-time visualization capabilities of \systemName enhanced their creative freedom and confidence in the final product.

